Optimized Custom Dataset for Efficient Detection of Underwater Trash

Accurately quantifying and removing submerged underwater waste plays a crucial role in safeguarding marine life and preserving the environment. While detecting floating and surface debris is relatively straightforward, quantifying submerged waste presents significant challenges due to factors like light refraction, absorption, suspended particles, and color distortion. This paper addresses these challenges by proposing the development of a custom dataset and an efficient detection approach for submerged marine debris. The dataset encompasses diverse underwater environments and incorporates annotations for precise labeling of debris instances. Ultimately, the primary objective of this custom dataset is to enhance the diversity of litter instances and improve their detection accuracy in deep submerged environments by leveraging state-of-the-art deep learning architectures.

==> dataset.tex <==
\section{Dataset} \label{sec:DS}  {
 \subsection {\textbf{Need for a custom dataset}}  {
Several datasets such as JAMSTEC, J-ED, TrashCAN 1.0 , Trash-ICRA19, etc are publicly available to use but the shortcoming of these datasets is that they are highly domain specific and adapted to the environment they were collected in. Current studies towards automatic waste detection are hardly comparable due to the lack of benchmarks and widely accepted standards regarding the used metrics and data \cite{MAJCHROWSKA2022274}. This exponentially reduces a model’s robustness as any deep learning model trained on these datasets will be highly adapted to the specifics and noise of the environment. To solve this, we have created an amalgamated, self-annotated dataset consisting of three classes which would prove to be the most useful for classifying the submerged debris which are Trash, Rover and Bio. With the help of the Bio class, we can also get an aspect of the marine life in the environment and how much has trash affected the marine life relative to nearby environments. The Rover class helps differentiate the rover from being misclassified as trash in some input imagery and finally, the trash class is used to detect and quantify the amount of trash found in the input image/video. The dataset was curated by first collecting inputs from various open-source datasets and videos across various countries with varying ocean environments. After collecting, manual annotation of marine debris in frames of images was done with a focus on selecting images with tricky object detection conditions like occlusion, noise, and illumination. The annotations were done with the help of a free tool \cite{7139973} to give rise to the final dataset, which comprised of 9625 images. 
}
\subsection{\textbf{Data Preparation}}  {

Before beginning, a comparison of all the existing datasets was performed (Figure 1) \cite{https://doi.org/10.48550/arxiv.2105.06808} in order to identify their limitations and therefore  create a custom dataset that would solve all of these shortcomings and make the model more robust. Our dataset was thereby termed Underwater-CDD which stands for Underwater-Curated-Debris-Detection. 

\input{datatable.tex}
\begin{figure}[h!]
\centering
  \includegraphics[width=.8\linewidth]{ss (1).png}
  \caption{Representative pictures from various datasets that were used
}
\end{figure}
\input{table2.tex}

A Deep learning analysis was also performed on these pre-existing datasets which can be viewed on this paper's source repository.\href{https://github.com/karanwxliaa/Underwater-Trash-Detection/tree/main/Custom\%20Models\%20on\%20Public\%20Datasets}{^2.} As suggested, the models performed well on training but when tested on unseen data from a slightly varying environment, it failed to detect the classes accurately.

The proposed data comprised of bounding box labels as well as image annotations. The proposed dataset UCDD is availabe in more than 10 different formats and can be imported directly for different algorithms to work on it.

The dataset was prepared using the subsequent steps.  
\begin{enumerate}


\item \textbf{Data collection}: The input images were selectively picked manually, comprising of different environments from different regions across the world.  

\item \textbf{Self-annotation}: The raw images without any annotations were then annotated respectively and various dataset’s annotations were merged and renamed into three final categories, Trash, Rov and Bio which stands for underwater debris, rover (autonomous vehicle) and biological marine life respectively. 

\item \textbf{Preprocessing}: These images were then rescaled to 416x416. A total of 26 classes were dropped and mapped into the final 3 classes. Clear water images that comprised of no annotations were also added to make the model more robust towards different enviornments. The dataset was further improved by randomly distorting the brightness and saturation of the images using PyTorch's built-in Transforms augmentation tool. This was done in order to mitigate the effects of the model generalizing towards undesirable features and to replicate variable underwater conditions such as illumination, occlusion, and coloring. 
\end{enumerate}

The total dataset consisted of 9625 images which were split into approximately 7300 for training, 1800 for validation and 473 for test.\\
The Labels of the dataset were as follows:
\begin{itemize}
  \item \textbf{Trash}: All sorts of marine debris (plastics, metals, etc).
  \item \textbf{Bio}: All naturally occurring biological material, marine life, plants, etc.
  \item \textbf{Rover}: Parts of the rover such as a robotic arm, sensors, or any part of the AUV to avoid misclassification.
\end{itemize}
}
}

==> includes.tex <==
%% ---------------------------
%% If you have other packages or command definitions you'd like to
%% include, write them there
%% ---------------------------
\usepackage{amsmath,amsfonts,amssymb}

%% Note: the subfig package is incompatible with the "unfixed" version
%% of the LIPICS class. It works here only because PaperShell includes
%% a fixed version --which is not the official version.
\usepackage{subfig}

%% We put one here: this is a dummy command for LaTeX, used to
%% tell Aspell to skip checking the spelling of what's inside
%% Usage: I like the word \nospellcheck{kwyjibo}
\newcommand{\nospellcheck}[1]{#1}

%% --------------------------
%% Personalized todo notes
%% --------------------------
\usepackage{xcolor}
\usepackage{todonotes}
%\newcommand{\todosylvain}[1]{\todo[inline,caption={},color=cyan]{\sf\small \textbf{@Sylvain:} #1}}
%\newcommand{\todoalex}[1]{\todo[inline,caption={},color=pink]{\sf\small \textbf{@Alex:} #1}}
%\newcommand{\todosebastien}[1]{\todo[inline,caption={},color=lime]{\sf\small \textbf{@Sébastien:} #1}}
%\newcommand{\todomichael}[1]{\todo[inline,caption={},color=lime]{\sf\small \textbf{@Michaël:} #1}}
%\newcommand{\todotous}[1]{\todo[inline,caption={},color=yellow]{\sf\small #1}}
%\newcommand{\todoedmond}[1]{\todo[inline,caption={},color=lime]{\sf\small \textbf{@Edmond:} #1}}

%% --------------------------
%% Placeholder for figure
%% --------------------------
\newcommand{\imagevide}{\framebox(200,200){IMAGE}}

%% --------------------------
%% Alter some LaTeX defaults for better treatment of figures:
%% See p.105 of "TeX Unbound" for suggested values.
%% See pp. 199-200 of Lamport's "LaTeX" book for details.
%% --------------------------
%% Parameters for all pages
\renewcommand{\topfraction}{0.9}	% max fraction of floats at top
\renewcommand{\bottomfraction}{0.8}	% max fraction of floats at bottom

%% Parameters for TEXT pages (not float pages)
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}                 % 2 may work better
\setcounter{dbltopnumber}{2}                % for 2-column pages
\renewcommand{\dbltopfraction}{0.9}         % fit big float above 2-col. text
\renewcommand{\textfraction}{0.07}          % allow minimal text w. figs

% Parameters for FLOAT pages (not text pages)
\renewcommand{\floatpagefraction}{0.7}      % require fuller float pages
% N.B.: floatpagefraction MUST be less than topfraction !!
\renewcommand{\dblfloatpagefraction}{0.7}   %require fuller float pages

%\newtheorem{example}{Example}

==> methodology.tex <==
 \section{Methodology}  {{{
With recent advancement in Computer vision technologies and algorithms, this section proposes latest debris detection and classification models followed by benchmarks for the proposed dataset and thereby statistically evaluating the training metrics. 

 \subsection{\textbf{Object Detection }}  {
The various architectures selected for this project were selected from the most latest, efficient, and successful object detection networks in use currently. Each has its own set of advantages and disadvantages, with different levels of accuracy, execution speeds, and other metrics. \\
We used several state-of-the-art neural network architectures like YOLOv8n (nano), YOLOv7, YOLO v6s, YOLO v5s, YOLO v4 Darknet using their respective repositories and also trained a custom FasterRCNN with Inception v2, masked RCNN.  
 }
 \subsection{\textbf{GPU Hardware}}  {
 In this project we have utilized Nvidia K80 GPU with a memory of 12GB and a memory clock rate of 0.82GHz. This GPU was released in the year 2014 with 2 CPU cores and 358gb disk space. 
 }

\subsection{\textbf{Models used}}  {
In this section we discuss about the latest models used and produced results. 

\subsubsection{\textbf{You Only Look Once (YOLO)}}  {
You Only Look Once, or YOLO, is a popular object detection technique that can recognize multiple items in a real-time video or image. In one evaluation, it utilizes a single neural network to predict bounding boxes and class probabilities straight from complete image. Because of this approach, YOLO is faster and more accurate than other object detection systems. 
\begin{itemize}
  \item \textbf{YOLOv8n \cite{yolov8} (nano)}: Leveraging the advancements of previous YOLO versions, the YOLOv8 model offers a faster and more accurate unified framework for training models, with the YOLOv8 Nano being the fastest and smallest among the available models. However, due to ongoing development, the YOLOv8 model exhibited various technical bugs, resulting in a weaker performance than expected.
  \item \textbf{YOLOv7 \cite{https://doi.org/10.48550/arxiv.2207.02696} (tiny/W6)}: The YOLOv7 algorithm outperforms its older versions in terms of speed and accuracy. It requires significantly less hardware than conventional neural networks and can be trained much more quickly on small datasets with no pre-learned weights
  \item \textbf{YOLOv5s \cite{glenn_jocher_2022_7347926} and YOLOv6s \cite{https://doi.org/10.48550/arxiv.1512.03385} (small)}: Both of these algorithms have similar performances and results.
\end{itemize}
}
\subsubsection{\textbf{Faster RCNN}}  {
Faster RCNN \cite{NIPS2015_14bfa6bb} is an improvement on R-CNN \cite{6909475} that introduces a Region Proposal Network (RPN) to make the whole object detection network end-to-end trainable. The RPN uses the last convolutional feature map to produce region proposals, which is then fed to the fully connected layers for the final detection. The original implementation uses VGG-16 \cite{simonyan2014deep} for feature extraction; we use the Inception v2 \cite{7780677} as feature extractor instead because it is known to produce better object detection performance in standard datasets \cite{tensorflowmodelgarden2020}.  Although it misidentifies patches in the background as objects which is due to its inability to see large contexts. When comparing generalization errors, YOLO algorithms surpass R-CNN because they produce a lower generalization error than R-CNN. In comparison to the YOLO algorithms, faster R-CNN also exhibited slightly less localization errors at the cost of higher computational needs and a slower speed. 
}
\subsubsection{\textbf{Mask RCNN}}  {
Mask R-CNN is a subset of Faster R-CNN that combines ResNet \cite{https://doi.org/10.48550/arxiv.1512.03385} with FPN as a feature extraction network to generate the feature map from the input image using a multi-layer convolutional feature extraction. The Region Proposal Network (RPN) is then utilized to produce proposals of region for the objects. Additionally, the detection head and mask head detect objects and segment instances. The algorithm is divided into two sections: detection and instance segmentation. 
However, in complicated maritime situations, Mask R-CNN suffers from problems caused by external variables such as distracting objects and inadequate image resolution. The key issues are difficulty while extracting object features and the low attention to objects for detection. 
}}
\subsubsection{\textbf{Evaluation metrics}}  {
After the model has been trained, we utilize the testing and validation datasets, which comprise images that are mutually exclusive from the training dataset, as input to analyze the network's accuracy. The model generates a bounding box around correctly recognized items with a confidence value of.50 or higher. The amount of true positive bounding boxes drawn around marine plastic waste and true negatives serves as the basis for evaluation. \\

The following performance metrics were used to generate results: 
\begin{itemize}
  \item \textbf{True positive and True negative values.}
  \item \textbf{Precision and Recall:} Reflects whether the model predicted debris in the input image.
  \[Recall = TP/(TP+FN)\]
  \[Precision = TP/(TP+FP)\]
  
  \item \textbf{Mean Average Precision:} – Determines how frequently the network can identify plastic in a set of photos. After gathering the true and false positive data, use the Intersection over Union (IoU) formula to build a precision-recall curve: 
 \[
 IOU = \mathlarger{ \frac{B Box_{pred}  \cap B Box_{GroundTruth}}{B Box_{pred}  \cup B Box_{GroundTruth}}}
 \]

Where $\mathlarger{B Box_{Predicted}}$ and $\mathlarger{B Box_{Groundtruth}}$ are the expected areas under the curve for predicted and ground truth bounding boxes. To maximize accuracy, a high threshold for confidence and IoU must be specified, with a correct prediction, indicated by the threshold being exceeded. After that, the mAP can be calculated by integrating the precision-recall curve. obtained by integrating the precision-recall curve \cite{10.1007/978-3-642-40994-3_29}:
\[
\mathlarger{mAP = \int_{0}^{1} p(x) dx}
\]
 \item \textbf{GPU Speed (ms/IMG):} – Refers to the rate at which the network can perform inferences for detecting and identifying marine plastic debris within an input image.
\end{itemize}
}
 }}}


==> midamble.inc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This file was autogenerated by PaperShell v2.6.1 on 2023-02-03 13:51:10
%% https://github.com/sylvainhalle/PaperShell
%% DO NOT EDIT!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibliographystyle{elsarticle-num}

\section*{References}


==> results.tex <==
 \section{Results}  {
\subsection{\textbf{Evaluating results}}{
The results for debris localization on our mixed, curated dataset UCDD overtakes prior research that employed individual datasets. Individual components of both the two frameworks were tested by performing exhaustive research on publicly available waste data in various contexts: clean waters, in natural or lakes/ponds surroundings, and ocean beds. The wide range of baseline results for different contexts and diverse object dimensions will aid other researchers in future investigations in this field. The tested models also have high average precision, mAP, and F1 scores in comparison to their inference speed.\\\\
The results of a comprehensive research comparing several architectural networks is shown in the Table.~\ref{tab:results}
\input{table3.tex}\\
These trade-offs indicate that the outcomes reported in this study better reflect long-term performance in a broader range of marine conditions, allowing for a more comprehensive evaluation of the object identification model's performance in the field. \\The study's findings indicate that YOLOv5-Small and YOLOv6s both achieve strong debris localization metrics in real-time detection of epipelagic plastic. Nevertheless, YOLOv7 yields a notably higher F1 score despite a slight reduction in inference performance. 

\\
\begin{figure}[h!]
\centering
  \includegraphics[width=.8\linewidth]{v5v7compare.png}
  \caption{Results comparing Precision \& Recall metrics between YOLOv5 \& YOLOv7 models}
\end{figure}\\

\\In addition to this, advanced algorithms within the same family (namely YOLOv5x, v7E6E, v8x) were also assessed which yielded similar outcomes. The decision was made to select the nano/small/tiny network architecture as it demonstrated the highest performance in evaluations, possessed a smaller parameter count, and required less computational power.\\These algorithms also surpassed the classic Faster-RCNN and Mask-RCNN algorithms as they proved to have a much faster speed and a much higher F1 score.
\begin{figure}[h!]
\centering
  \includegraphics[width=.8\linewidth]{cm.png}
  \caption{Confusion matrix for the proposed model}
\end{figure}
The model's performance in real-world deployments produced a similar result, thus resulting in only minor deviations between the evaluation results presented in Table.3 and those obtained in a near-real-time environment. \\The proposed research may function as a fundamental baseline and a benchmark for subsequent research pertaining to the identification and categorization of underwater debris. 
}
\subsection{\textbf{Visualising results}}{
As part of its image processing, the network captures two important data points in arrays:\\ \textbf{Scores}, which reflect the degree of certainty for the predicted boxes, and the total number of \textbf{Detections} made on the image.\\
In order to render the bounding boxes on the images, the network converts the normalized coordinates to image coordinates, utilizing a specific equation.
\[ 
ImgCord_{k} = BoxScore_{i}^{j} \ast Width 
\]
where $k$ belongs to the top, down, right and left corners, $i$ is the box index, $j$ $\epsilon$  ${0, 1, 2, 3}$, and $Width$ is the image width. In the test images, these image coordinates were utilized to illustrate the results of predicted bounding boxes.\\
The results below were obtained on the test dataset described in the\\ \hyperref[sec:DS]{^3 Dataset Section,} which was designed to be challenging to the models and to provide a true-to-life representation of how a marine debris detector would have to operate. 
\begin{figure}[h!]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{rcnnbatch.png}
  \caption{Batch results for Faster-RCNN}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{yolobatch.png}
  \caption{Batch results for YOLO models}
  \label{fig:sub2}
\end{subfigure}
\caption{Comparison between the detection outputs of RCNN \& YOLO models.}
\label{fig:test}
\end{figure}
In addition to analyzing the models using our test set, we also subjected each network to two additional videos, as illustrated in Figure 4. One of the videos shown in Figure 5 was a viral footage of ocean waste captured in Bali \cite{yt}, which presented a unique and previously unseen visual context compared to our training set. Despite the significant challenges posed by this video to all our detectors, our models were able to provide promising detections. 
\begin{figure}[h!]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{v5v7bali.png}
  
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{v5v7bali2.png}
  
  \label{fig:sub2}
\end{subfigure}
\caption{Performance on new, unseen test data using the two best-performing models}
\label{fig:test}
\end{figure}

 
}

 }

==> table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
{\ul \textbf{Dataset}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Total\\ Classes\end{tabular}} &
  {\color[HTML]{2E2E2E} {\ul \textbf{Bio}}} &
  {\color[HTML]{2E2E2E} \textbf{\begin{tabular}[c]{@{}c@{}}Paper\\ \&\\ Glass\end{tabular}}} &
  {\color[HTML]{2E2E2E} \textbf{\begin{tabular}[c]{@{}c@{}}Metals \\ \&\\ Plastic\end{tabular}}} &
  {\color[HTML]{2E2E2E} \textbf{\begin{tabular}[c]{@{}c@{}}Other\\ Non-\\ recyclable\end{tabular}}} &
  {\ul \textbf{Unknown}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Total\\ Images\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Environmental\\ Conditions\end{tabular}} \\ \hline
Trash ICRA-19 &
  3 &
  1966 &
  - &
  5051 &
  - &
  - &
  6148 &
  \begin{tabular}[c]{@{}c@{}}Normal\\ Underwater\end{tabular} \\ \hline
{\color[HTML]{2E2E2E} TrashCan 1.0} &
  3 &
  {\color[HTML]{2E2E2E} 1009} &
  {\color[HTML]{2E2E2E} -} &
  {\color[HTML]{2E2E2E} 2163} &
  {\color[HTML]{2E2E2E} -} &
  180 &
  7212 &
  \begin{tabular}[c]{@{}c@{}}Normal\\ Underwater\end{tabular} \\ \hline
{\color[HTML]{2E2E2E} TrashNet} &
  6 &
  {\color[HTML]{2E2E2E} -} &
  {\color[HTML]{2E2E2E} 1300} &
  {\color[HTML]{2E2E2E} -} &
  {\color[HTML]{2E2E2E} -} &
  - &
  2527 &
  Clear Background \\ \hline
{\color[HTML]{2E2E2E} Google search} &
  - &
  {\color[HTML]{2E2E2E} 92} &
  {\color[HTML]{2E2E2E} 250} &
  {\color[HTML]{2E2E2E} -} &
  {\color[HTML]{2E2E2E} -} &
  366 &
  1320 &
  Varying \\ \hline
{\color[HTML]{2E2E2E} Extended TACO} &
  28 &
  {\color[HTML]{2E2E2E} 70} &
  {\color[HTML]{2E2E2E} 1190} &
  {\color[HTML]{2E2E2E} 6060} &
  {\color[HTML]{2E2E2E} 2800} &
  150 &
  1500 &
  Wild Waste \\ \hline
{\color[HTML]{2E2E2E} Drinking waste} &
  4 &
  {\color[HTML]{2E2E2E} -} &
  {\color[HTML]{2E2E2E} 1160} &
  {\color[HTML]{2E2E2E} 3600} &
  {\color[HTML]{2E2E2E} -} &
  - &
  9640 &
  \begin{tabular}[c]{@{}c@{}}Clear Conditions,\\ Cans \& Bottles\end{tabular} \\ \hline
Classify-waste &
  3 &
  160 &
  3900 &
  9660 &
  2800 &
  520 &
  27500 &
  Varying \\ \hline
\end{tabular}%
}
\caption{Table comparing various classes of chosen datasets.} 
\end{table}

